Cold-Start Data Selection for Few-shot Language Model Fine-tuning: A Prompt-Based Uncertainty Propagation Approach

Large Language Models have demonstrated remarkable few-shot performance, but the performance can be sensitive to the selection of few-shot instances. We propose PATRON, a new method that uses prompt-based uncertainty estimation for data selection for pre-trained language model fine-tuning under cold-start scenarios, i.e., no initial labeled data are available. In PATRON, we design (1) a prompt-based uncertainty propagation approach to estimate the importance of data points and (2) a partition-then-rewrite (PTR) strategy to promote sample diversity when querying for annotations. Experiments on six text classification datasets show that PATRON outperforms the strongest cold-start data selection baselines by up to 6.9%. Besides, with 128 labels only, PATRON achieves 91.0% and 92.1% of the fully supervised performance based on vanilla fine-tuning and prompt-based learning respectively. Our implementation of PATRON is available at \url{https://github.com/yueyu1030/Patron}.

==> 03-exp-case-study.tex <==
\section{Runtime Analysis.}

\label{sec:time}
Table~\ref{tab:time} shows the time in one active learning round of {\ours} and  baselines. Here we highlight that the additional time for region-aware sampling and momentum-based memory bank is \emph{rather small} compared with the inference time.
Among all baselines, we find that the running time of clustering-based method is faster than the original reported time in the paper. 
This is because we use FAISS~\cite{FAISS} instead of SKLearn~\cite{pedregosa2011scikit} for clustering, which accelerates the clustering step significantly.
Also, we find that BALD and REVIVAL are not so efficient. For BALD, it needs to infer the uncertainty of the model by passing the data to model with multitple times. Such an operation will make the total inference time for PLMs very long.
For REVIVAL, we find that calculating the adversarial gradient needs extra forward passes and backward passes, which could be time-consuming for PLMs with millions of parameters\footnote{The original model is proposed with CV tasks and they use ResNet-18 as the backbone which only contains 11M parameters (around 10\% of the parameters of Roberta-base).}.

% \paragraph{Diversity and Uncertainty Analysis.}

\section{Limitations}
First, since our focus is on fine-tuning pre-trained language models, we use the representation of \texttt{[CLS]} token for classification. 
In the future work, we can consider using prompt tuning~\cite{gao2021making,schick-schutze-2021-exploiting}, a more data-efficient method for adopting pre-trained language models on classification tasks to further promote the efficiency. 
Also, due to the computational resource constraints, we do not use larger pre-trained language models such as RoBERTa-large~\cite{liu2019roberta} which shown even better performance with only a few labels~\cite{du-etal-2021-self}.
Last, apart from the text classification task, we can also extend our work into other tasks such as sequence labeling and natural language inference.
% labeling 
% we can combine {\ours}
% design more advanced denoising
% methods for self-training, such as sample reweighting (Yu et al., 2021; Wang et al., 2021); Second,
% we can design better policies that are more suitable for ATM to further improve the fine-tuning
% performance of LMs; Third, it is also desirable
% to combine the prompt-tuning (Gao et al., 2021;
% Schick and Schütze, 2021) with ATM to improve
% the label efficiency. Last but not least, we plan
% to adopt ATM 

\section{Case Study}
Here we give an example of our querying strategy on AG News and Pubmed dataset for the 1st round of active self-training process in  figure~\ref{fig:case_study}. Note that we use t-SNE algorithm~\cite{tsne} for dimension reduction, and the black triangle stands for the queried samples while other circles stands for the unlabeled data. 
Different colors stands for different classes. From the comparision, we can see that the existing uncertainty based methods such as Entropy and CAL, are suffered from the issue of limited diversity. However, when combined with {\ours}, the diversity is much improved. Such results, compared with the main results in figure~\ref{fig:main}, demonstrate the efficacy of {\ours} empirically.

\begin{figure*}[t]
    \vspace{-2mm}
    %\begin{small}
        \centering
        \subfigure[AG News, Entropy]{
            \includegraphics[width=0.48\textwidth]{figure/agnews_entropy_50.pdf}
            \label{fig:param_beta}
        }\hspace{-2mm}
        \subfigure[AG News, {\ours} w/ Entropy]{
            \includegraphics[width=0.48\textwidth]{figure/agnews_region_entropy_50.pdf}
            \label{fig:param_K}
        }\hspace{-2mm}\vspace{-2ex}
                 \subfigure[AG News, CAL]{
            \includegraphics[width=0.48\textwidth]{figure/agnews_cal_50.pdf}
            \label{fig:acc_pseudo}
        }\hspace{-2mm}
        \subfigure[AG News, {\ours} w/ CAL]{
    \includegraphics[width=0.48\textwidth]{figure/agnews_region_cal_50.pdf}
            \label{fig:entropy_m}
        }
       \vspace{-2ex}
       \subfigure[Pubmed, Entropy]{
            \includegraphics[width=0.48\textwidth]{figure/pubmed_entropy_40.pdf}
            \label{fig:param_beta}
        }\hspace{-2mm}
        \subfigure[Pubmed, {\ours} w/ Entropy]{
            \includegraphics[width=0.48\textwidth]{figure/pubmed_region_entropy_40.pdf}
            \label{fig:param_K}
        }\hspace{-2mm}
                 \subfigure[Pubmed, CAL]{
            \includegraphics[width=0.48\textwidth]{figure/pubmed_cal_40.pdf}
            \label{fig:acc_pseudo}
        }\hspace{-2mm}
        \subfigure[Pubmed, {\ours} w/ CAL]{
    \includegraphics[width=0.48\textwidth]{figure/pubmed_region_cal_40.pdf}
            \label{fig:entropy_m}
        }
        \caption{Visualization of the querying strategy of {\ours}.}\label{fig:case_study}
         \vspace{-3ex}
    %\end{small}\
\end{figure*}


==> main_table.tex <==
\begin{table*}[t!]
    \centering
    \caption{The main result of classification accuracy on different datasets with various labeled samples. Note that \colorbox{red!15!white}{red} stands for the result of self-training methods, \colorbox{yellow!15!white}{yellow} stands for active learning methods, \colorbox{green!15!white}{green} stands for semi-supervised self-training methods, and \colorbox{blue!15!white}{blue} stands for the result of {\ours}. Best view in color.}
    \label{tab:main}
    \begin{adjustbox}{max width=0.9\textwidth}
% Please add the following required packages to your document preamble:
\begin{tabular}{c|c|l|ccccccccc}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\bf Dataset}} & \multicolumn{1}{c|}{\multirow{2}{*}{\bf Line}} &  \multicolumn{1}{c|}{\multirow{2}{*}{\bf Method}}  &  \multicolumn{9}{c}{\bf \# of labels}                          \\ \cline{4-12} 
\multicolumn{1}{l|}{}                         & \multicolumn{1}{c|}{}      & \multicolumn{1}{c|}{}                        & 200 & 300 & 400 & 500 & 600 & 700 & 800 & 900 & 1000 \\ \midrule
\multirow{23}{*}{SST-2}                        & 1 & Finetune                            &   85.8\std1.0  &  86.6\std0.8   &    87.5\std0.6  & 88.0\std0.3    & 88.9\std0.3    &    89.2\std0.2 & 90.1\std0.6    & 90.1\std0.3    & 90.0\std0.2                              \\ \cline{2-11} 
&  2 &Self-training~\shortcite{lee2013pseudo}                                &   \st{86.5\std0.4}  &   \st{87.5\std0.5}  &   \st{87.7\std0.2}  & \st{88.2\std0.3}    &  \st{88.6\std0.5}   &  \st{89.2\std0.4}   &  \st{90.0\std0.5}   &  \st{90.4\std0.4}   &   \st{90.1\std0.4}                      \\
& 3 & UST~\shortcite{mukherjee2020uncertainty,rizve2021in}                                            & \st{88.0\std0.8}    &  \st{88.1\std0.9}   &  \st{89.1\std0.6}   &  \st{90.1\std0.5}   &  \st{89.2\std0.3}   &  \st{90.1\std0.4}   & \st{90.5\std0.6}    &  \st{90.7\std0.5}   & \st{90.7\std0.4}                            \\ \cline{2-11} 
& 4 &Entropy~\shortcite{holub2008entropy}                                     & \al{85.2\std0.4}    & \al{86.7\std0.5}     & \al{87.6\std0.3}     & \al{88.3\std0.3}      &    \al{88.9\std0.4}  & \al{89.2\std0.6}     &   \al{89.5\std0.3}  &    \al{90.1\std0.4} & \al{89.6\std0.3}                               \\
% & \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}                                       &   \ssal{89.2\std0.9}  &   \ssal{87.8\std0.8}  & \ssal{88.2\std0.7} & \ssal{88.1\std0.3}     &  \ssal{90.2\std0.3}   &  \ssal{90.5\std0.4}   & \ssal{90.8\std0.3}    & \ssal{91.1\std0.3}    & \ssal{90.6\std0.4}                              \\
& 5 &\ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}  &                       \ssal{87.0\std0.4} & \ssal{88.4\std0.3} &  \ssal{88.7\std0.3}   & \ssal{88.9\std0.1}     &  \ssal{89.5\std0.2}   &  \ssal{89.4\std0.1}   & \ssal{89.3\std0.5}    & \ssal{90.0\std0.5}        & \ssal{89.9\std0.2}                              \\
& 6 & \ \ \ \ \  w/ {\ours}    & \bf \our{88.2\std{0.4}}     & \our{88.6\std0.3}   & \our{89.6\std0.3}     & \our{90.0\std0.2}    & \bf  \our{90.6\std0.2}   & \our{90.8\std0.3} & \our{90.7\std0.1}     &    \our{91.2\std0.2} & \our{91.1\std0.1}                               \\
 &7 & BALD~\shortcite{gal2017deep,balm}                         & \al{86.3\std0.2}     &  \al{87.7\std0.3}   & \al{88.1\std0.2}    & \al{87.2\std0.4}    & \al{88.9\std0.5} & \al{89.0\std0.2}     &\al{88.8\std0.3}  & \al{90.0\std0.3}    & \al{89.2\std0.5}     \\
%  &  \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}                                       &   \ssal{89.2\std0.9}  & \ssal{88.4\std0.3}    & \ssal{89.5\std0.4}    & \ssal{89.0\std0.2}    & \ssal{90.4\std0.2}    &\ssal{90.5\std0.4}     & \ssal{89.9\std0.3}    &\ssal{90.0\std0.2}     & \ssal{90.0\std0.2}                               \\
& 8 & \ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}    & \ssal{87.2\std0.4}     & \ssal{87.6\std0.2}    &  \ssal{88.4\std0.2}   &  \ssal{88.5\std0.1}   & \ssal{88.7\std0.2}     & \ssal{89.6\std0.4}    & \ssal{89.9\std0.3}    & \ssal{89.8\std0.2}    & \ssal{89.8\std0.1}                           \\
& 9 &  \ \ \ \ \ w/ {\ours}  & \our{87.1\std0.5}    & \our{88.2\std0.3}     &  \our{88.3\std0.3}    & \our{88.6\std0.2}    & \our{89.1\std0.2}     & \our{89.8\std0.3}    & \our{89.7\std0.2}     &    \our{90.3\std0.2} & \our{90.3\std0.1}                               \\
&10 & ALPS~\shortcite{yuan-etal-2020-cold}              & \al{86.3\std0.7}    & \al{86.6\std0.4}     & \al{87.4\std0.6}    &  \al{87.9\std0.5}   & \al{87.7\std0.4}    &    \al{88.5\std0.5} &  \al{89.1\std0.3}    &  \al{89.6\std0.2}   & \al{89.7\std0.2}                       \\
% &  \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}            & \ssal{87.3\std0.5}    & \ssal{}     &     &     &     &      &     &     &                           \\
& 11 & \ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}      & \ssal{87.3\std0.3} &  \ssal{87.1\std0.2}  &    \ssal{88.1\std0.4}  & \ssal{88.3\std0.2} &   \ssal{89.1\std0.5}  & \ssal{88.5\std0.2}    &  \ssal{89.4\std0.6}   & \ssal{89.6\std0.3}    & \ssal{90.0\std0.1}                           \\
& 12 &  \ \ \ \ \  w/ {\ours}  &    \our{87.5\std0.2} & \our{89.0\std0.3}     & \our{88.8\std0.1}    & \our{88.9\std0.1}     &  \our{89.0\std0.2}   &  \our{89.7\std0.3}    & \our{90.0\std0.2}    &    \our{90.5\std0.2} & \our{91.0\std0.1}                              \\
 &13 & BADGE~\shortcite{badge}  & \al{86.3\std0.7}    & \al{87.7\std0.2}    &  \al{88.0\std0.2}   & \al{88.3\std0.2}    & \al{88.2\std0.6}    & \al{88.9\std0.6}   &    \al{89.5\std0.5} & \al{89.7\std0.3}         &  \al{89.9\std0.4}                         \\
%  &  \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}                                       &     &     &         &     &     &     &     &     &                           \\
&14 &  \ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}       &  \ssal{86.9\std0.4}       & \ssal{86.7\std0.5}    &      \ssal{88.1\std0.4}  & \ssal{88.3\std0.2}    &  \ssal{87.9\std0.3}  &   \ssal{89.2\std0.2}  & \ssal{89.3\std0.3}     &    \ssal{89.3\std0.1} & \ssal{89.8\std0.3}                   \\
& 15 &  \ \ \ \ \  w/ {\ours}    & \our{87.4\std0.2}     & \our{87.9\std0.1}     & \our{88.6\std0.1}     & \our{88.7\std0.1}    & \our{88.6\std0.2}    & \our{89.2\std0.1}    & \our{89.6\std0.2}     & \our{90.1\std0.3}     &   \our{90.9\std0.2}                            \\
 &16 & CAL~\shortcite{margatina2021active}   & \al{86.4\std0.3}    & \al{87.6\std0.5}    & \al{88.4\std0.3}    &    \al{87.8\std0.2} &  \al{88.3\std0.2}   &    \al{89.1\std0.4}     & \al{89.3\std0.4}     &   \al{89.8\std0.2}  & \al{90.2\std0.3}                           \\
%  &  \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}                                       &     &     &     &         &     &     &     &     &                           \\
& 17 & \ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}             & \ssal{87.8\std0.4}     & \ssal{88.0\std0.1}  &  \ssal{89.2\std0.3}   & \ssal{89.6\std0.1}   & \ssal{89.5\std0.2}     & \ssal{90.2\std 0.2}    & \ssal{90.5\std 0.3}    &    \ssal{90.8\std 0.2} & \ssal{90.6\std 0.2}                          \\
& 18 &  \ \ \ \ \  w/ {\ours}   & \our{87.2\std0.3}     & \bf \our{89.5\std0.5}    & \bf \our{90.1\std0.2}     &\bf  \our{90.3\std0.3}    & \our{90.5\std0.1}    & \bf \our{90.9\std0.2}    & \bf \our{90.8\std0.3}    &  \bf   \our{91.3\std0.1} & \bf \our{91.5\std0.1}                               \\ \midrule
 \multirow{18}{*}{AG News}     &19 & Finetune         &    {87.6\std0.2} & {88.3\std0.3}    & {88.4\std0.2}     & 89.0\std0.1    &  88.8\std0.3    &     88.6\std0.4 &  88.9\std0.5  &   89.3\std0.3           &  89.6\std0.4              \\ \cline{2-11} 
&20 & Self-training~\shortcite{lee2013pseudo}                            &  \st{87.8\std0.1} & \st{88.3\std0.3}    & \st{88.8\std0.3}     & \st{89.3\std0.4}    &  \st{89.9\std0.3}    &     \st{89.8\std0.6} &  \st{90.0\std0.4}  &   \st{90.2\std0.2}     &  \st{90.1\std0.3}      \\
&21 & UST~\shortcite{mukherjee2020uncertainty,rizve2021in}                                           & \st{89.3\std0.5}    &    \st{89.4\std0.4}  & \st{89.2\std0.5}    & \st{89.6\std0.2}    &  \st{90.1\std0.7}   & \st{90.3\std0.3}    & \st{90.2\std0.5}    &  \st{90.6\std0.4}   & \st{90.8\std0.3}                               \\ 
\cline{2-11} 
&22 & Entropy~\shortcite{holub2008entropy}  &   \al{87.7\std0.3} & \al{88.5\std0.3}  & \al{89.4\std0.4}   & \al{89.6\std0.6}    &    \al{89.3\std 0.5}  &  \al{89.4\std 0.3}   & \al{89.6\std 0.3} & \al{89.8\std 0.5}    & \al{90.0\std0.2}                \\
% &  \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}                                       &     &     &     &     &     &     &     &     &                           \\
& 23 & \ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}      & \ssal{88.0\std 0.2} & \ssal{89.1\std0.4}    &\ssal{88.8\std0.3}     &  \ssal{90.0\std0.5}   & \ssal{90.5\std0.2}    & \ssal{90.6\std0.3}    & \ssal{90.7\std0.1} & \ssal{90.7\std0.2}    & \ssal{90.8\std0.2}          \\
& 24 &  \ \ \ \ \  w/ {\ours}  &    \our{88.2\std0.4} & \bf \our{90.0\std0.3}   & \our{90.3\std0.2}    &    \our{90.3\std0.2} & \our{90.6\std0.4}    & \our{90.9\std0.3}    & \our{90.8\std0.2}    & \our{91.0\std0.4}    &       \our{91.4\std0.3}                   \\
 &25 & BALD~\shortcite{gal2017deep,balm}& \al{88.4\std0.2}    & \al{89.3\std0.4}    & \al{89.5\std0.2}    & \al{90.0\std0.3}    &  \al{89.9\std0.2}      &   \al{90.3\std0.1}  &     \al{90.5\std0.4} & \al{90.6\std0.5}    &  \al{90.5\std0.3}                         \\
%  &  \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}                                       &     &     &     &     &     &     &     &     &                           \\
&26 &  \ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}       & \ssal{88.9\std0.1}     &  \ssal{89.1\std0.4}   & \ssal{89.7\std0.2}   & \ssal{89.5\std0.4}    & \ssal{90.3\std0.3}    &  \ssal{90.4\std0.2}   & \ssal{90.6\std0.3}    &  \ssal{90.7\std0.1}   & \ssal{90.7\std0.2}                          \\
& 27 &  \ \ \ \ \  w/ {\ours}  &    \our{88.8\std0.2}  & \our{89.7\std0.1}    & \our{89.8\std0.5}  & \our{90.4\std0.2}    & \our{90.5\std0.3}    & \our{90.5\std0.4}    & \our{90.6\std0.2}    &  \our{90.8\std0.3}   & \our{91.1\std0.3}                          \\
& 28 &ALPS~\shortcite{yuan-etal-2020-cold}    & \al{87.7\std0.1}     & \al{87.8\std0.2}  & \al{87.9\std0.2}   & \al{89.2\std0.4}    &  \al{89.1\std0.3}   &  \al{89.2\std0.3}   & \al{89.1\std0.4}    & \al{89.6\std0.3} & \al{89.5\std0.2}       \\
% &  \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}                                       &     &     &     &     &     &     &     &                                \\
&29 &  \ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}     & \ssal{88.1\std0.2}    & \ssal{88.0\std0.3}    & \ssal{88.6\std0.5}    & \ssal{88.7\std0.2}    & \ssal{88.6\std0.4}    & \ssal{89.2\std0.3}    & \ssal{89.6\std0.1}    & \ssal{89.9\std0.4}      & \ssal{89.7\std0.3}                        \\
& 30 & \ \ \ \ \  w/ {\ours} &    \our{89.2\std0.4} & \our{88.8\std0.3}    &    \our{89.2\std0.3} & \our{89.0\std0.2}    &   \our{89.6\std0.3}   & \our{90.0\std0.2}    &  \our{89.8\std0.1}    &  \our{90.2\std0.3}    &  \our{90.4\std0.2}      \\
 &31 & BADGE~\shortcite{badge}   & \al{87.7\std0.2}     & \al{88.6\std0.4}  & \al{89.1\std0.2}   & \al{89.0\std0.1}    &  \al{89.0\std0.2}   &  \al{89.5\std0.3}   & \al{89.8\std0.2}    & \al{89.9\std0.1} & \al{90.0\std0.3}       \\
%  & \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}                                       &     &     &     &     &     &     &     &                              \\
&32 &  \ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}       &  \ssal{88.2\std0.3}   &  \ssal{88.4\std0.3}   &  \ssal{89.4\std0.4}   & \ssal{89.3\std0.5}    &  \ssal{89.9\std0.2}   & \ssal{89.6\std0.3}        &  \ssal{89.8\std0.2}   & \ssal{89.8\std 0.3} &      \ssal{90.1\std 0.4}                     \\
&33 &   \ \ \ \ \  w/ {\ours}       & \our{88.7\std0.3}    &    \our{88.9\std 0.5} &\our{89.3\std0.3}    & \our{89.2\std0.2}    & \our{89.6\std0.4}    &    \our{90.1\std0.3} &     \our{90.0\std0.4}& \our{90.1\std0.2}    &       \our{90.5\std0.2}                     \\
 &34 & CAL~\shortcite{margatina2021active}   & \al{88.6\std0.4}    &    \al{88.8\std 0.5} & \al{89.2\std0.1}    &  \al{89.8\std0.2}   &  \al{90.0\std0.1}   & \al{89.8\std0.3}    &    \al{90.5\std0.5} & \al{90.7\std0.4}    & \al{90.8\std0.4}                          \\
%  &  \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}                                       &     &     &     &     &     &     &     &     &                           \\
& 35 & \ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}        &\ssal{89.6\std0.2}     &  \ssal{89.8\std0.3}   &\ssal{90.0\std 0.1}     & \ssal{90.1\std0.4}    & \ssal{90.2\std0.2}    & \ssal{90.4\std0.3}    & \ssal{90.7\std0.4}    & \ssal{91.0\std0.2}    &      \ssal{91.2\std0.2}                     \\
& 36 &  \ \ \ \ \  w/ {\ours}     & \bf \our{89.4\std0.1}    & \our{89.9\std0.3}    & \bf \our{90.6\std0.5}    &\bf  \our{90.9\std0.4}    & \bf  \our{91.2\std0.3}   &\bf  \our{91.2\std0.2}    & \bf \our{91.5\std 0.3}    &  \bf   \our{91.8\std0.2} &   \bf  \our{91.9\std0.3}                       \\ \midrule
\multirow{18}{*}{Pubmed-RCT}        & 37 &Finetune   &    80.9\std0.2 &    81.2\std0.3 & 82.1\std0.6    & 82.6\std0.3    & 82.9\std 0.4    &    83.4\std0.3 & 83.6\std0.2    &   82.8\std0.5 & 82.9\std0.2                             \\ \cline{2-11} 
& 38 &Self-training~\shortcite{lee2013pseudo}    & \bf \st{81.6\std0.3}  & \st{81.7\std0.4}  &\st{83.0\std0.6}  & \st{82.6\std0.7} & \st{83.0\std0.4} & \st{83.1\std0.5}  & \st{83.4\std0.5} & \st{83.6\std0.3} & \st{83.1\std0.5} \\
& 39 &UST~\shortcite{mukherjee2020uncertainty,rizve2021in}                                          &  \st{81.3\std0.4}   & \st{81.5\std0.4}    &  \st{82.6\std0.5}   & \st{82.5\std0.3}    &\st{83.4\std0.5}     & \bf \st{83.9\std0.4}    &   \st{83.1\std0.5}    &  \st{83.8\std0.3}   & \st{83.4\std0.3}                          \\ \cline{2-11} 
& 40 &Entropy~\shortcite{holub2008entropy}   &   \al{80.0\std0.7}  &    \al{80.6\std0.4} & \al{81.5\std0.3}    &    \al{81.7\std0.2} & \al{82.3\std0.3}    &    \al{82.7\std0.4}      & \al{83.2\std0.1}    &   \al{83.1\std0.2}  & \al{82.6\std0.4}                          \\
% &  \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}                                      &   \ssal{12.1\std0.1}  &     &     &     &     &     &     &     &                              \\
&  41 &\ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}      & \ssal{80.9\std0.3}     & \ssal{80.4\std1.0}    & \ssal{81.2\std0.3}    & \ssal{82.9\std0.5}    &  \ssal{81.3\std0.4}   & \ssal{81.9\std0.3}    & \ssal{82.5\std0.2}    & \ssal{82.7\std0.3}    & \ssal{83.7\std0.5}        \\
& 42 &  \ \ \ \ \  w/ {\ours}   &  \our{81.5\std0.3}  & \our{82.1\std0.2}    & \our{82.6\std0.5}    & \our{82.5\std0.3}    & \our{82.9\std0.2}    & \our{82.7\std0.5}     & \our{83.7\std0.4}     & \our{83.6\std0.2}    & \our{84.3\std0.3}                           \\
 &43 & BALD~\shortcite{gal2017deep,balm}  & \al{80.2\std0.3}    & \al{81.2\std0.4}    & \al{81.2\std0.2}     & \al{80.9\std0.3}    & \al{81.9\std0.2}     & \al{81.8\std0.1}    & \al{82.2\std0.3}     &\al{82.4\std0.2}     & \al{82.6\std0.4}                             \\
%  &  \ \ \ \ \ w/ LP~\shortcite{simeoni2021rethinking}                                       &     &     &     &     &     &     &     &     &                             \\
& 44 & \ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}     & \ssal{80.9\std0.5}    &  \ssal{81.2\std0.3}   &   \ssal{81.6\std0.3}  & \ssal{81.5\std0.8}    & \ssal{82.4\std0.6} &   \ssal{82.5\std0.3}  &    \ssal{82.4\std0.2} &    \ssal{82.3\std 0.5} & \ssal{82.9\std0.4}                             \\
&45 &   \ \ \ \ \  w/ {\ours}        &\our{80.7\std0.4}     &  \our{81.3\std0.3}   & \our{82.1\std0.4}     &  \our{81.5\std0.6}   & \our{82.5\std0.5}    & \our{83.4\std0.4}    & \our{83.7\std0.3}    &    \our{83.8\std0.4} & \our{84.0\std0.3}                           \\
&46 & ALPS~\shortcite{yuan-etal-2020-cold}  & \al{80.1\std0.3}    & \al{81.6\std0.6}    & \al{81.9\std0.4}     & \al{82.5\std0.4}     & \al{82.5\std0.2}    &  \al{83.4\std0.4}    & \al{83.0\std0.3}     & \al{82.5\std0.5}     & \al{82.4\std0.3}                           \\
% &  \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}                                       &     &     &     &     &     &     &     &     &                           \\
&47 &  \ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}          &    \ssal{81.1\std0.3} & \ssal{82.0\std0.4}    &    \ssal{81.5\std0.6} &    \ssal{82.5\std0.3} &    \ssal{82.6\std0.1} & \ssal{83.0\std0.2}    & \ssal{83.2\std0.4}     & \ssal{82.5\std 0.3}    & \ssal{82.6\std0.2}   \\
& 48 & \ \ \ \ \  w/ {\ours}   & \our{81.4\std0.4} & \bf \our{82.3\std0.3}  & \bf \our{82.7\std0.5} &    \our{83.0\std0.2} & \our{82.9\std0.5}     & \our{83.5\std0.2}    & \our{82.4\std0.4}   &  \our{82.6\std0.3}   & \our{82.7\std0.5}  \\
 &49 & BADGE~\shortcite{badge}   & \al{80.9\std0.3} & \al{82.0\std0.6}   & \al{82.3\std0.3}     & \al{82.6\std0.6}     &  \al{82.0\std 0.5}   & \al{82.4\std0.3}     & \al{82.8\std 0.4}    & \al{82.6\std0.4}    &   \al{82.5\std0.3}                         \\
%  &  \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}                                       &     &     &     &     &     &     &     &     &                           \\
 & 50 & \ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}   & \ssal{81.1\std0.2}    &  \ssal{82.3\std0.2}   & \ssal{82.5\std0.3}    & \ssal{82.8\std0.2}    &  \ssal{82.7\std0.1}   &\ssal{83.0\std0.3}     &  \ssal{83.2\std0.4}   & \ssal{83.4\std0.3}    & \ssal{82.6\std0.2}                          \\
& 51 &  \ \ \ \ \  w/ {\ours}    & \our{81.2\std0.1}    & \our{82.1\std0.3}    &    \our{82.8\std0.4} & \our{83.3\std0.3}    & \our{83.1\std0.3}    & \our{83.0\std0.4}    &    \our{83.4\std0.3} & \our{83.2\std0.2}    & \our{83.5\std0.3}         \\
 & 52 &CAL~\shortcite{margatina2021active}      &     \al{81.0\std0.3} & \al{82.1\std0.1}    & \al{82.7\std0.2}    &  \al{82.9\std0.5}    & \al{83.1\std0.3}    & \al{83.2\std0.5}   & \al{83.7\std0.1} & \al{83.5\std0.2}    &  \al{83.6\std0.3}                          \\
%  &  \ \ \ \ \  w/ LP~\shortcite{simeoni2021rethinking}                                       &     &     &     &     &     &     &     &     &                            \\
&53 &  \ \ \ \ \   w/ ASSL~\shortcite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking}     & \ssal{81.4\std0.2}    &\ssal{81.5\std0.1}     &\ssal{82.5\std0.4}     &\ssal{83.1\std0.6}     & \ssal{82.8\std0.7}    & \ssal{83.0\std0.4}    & \ssal{83.6\std0.3}    &    \ssal{84.2\std0.2} &\ssal{84.3\std0.2}                            \\
& 54 &  \ \ \ \ \  w/ {\ours}     &\our{81.2\std0.3}     &\bf \our{82.3\std0.2}     &\our{82.6\std0.5}     & \bf \our{83.5\std0.3}     & \bf \our{83.5\std0.4}     &  \our{83.6\std0.2}   & \bf \our{83.9\std0.3}    & \bf \our{84.3\std0.5}    & \bf  \our{84.9\std0.3}                        \\ \bottomrule
\end{tabular}
    \end{adjustbox} 
\end{table*}


==> tables/main_prompt.tex <==


\begin{table*}[t]
% \resizebox{\linewidth}{!}{%
% \scalebox{0.57}{
\centering 
\renewcommand\arraystretch{0.75}
\fontsize{7.5}{9.5}\selectfont \setlength{\tabcolsep}{0.5em}
\resizebox{0.95\linewidth}{!}{%
\begin{tabular}{c|c|c|cc|cc|ccc|c}
% \Xhline{2\arrayrulewidth}
\toprule
% \multicolumn{9}{c}{\textbf{Entity Typing}}    \\ \Xhline{2\arrayrulewidth}
\bf    Task     & $c$ & \bf  Random & \bf Uncertainty & \bf CAL  & \bf BERT-KM &\bf  Coreset & \bf Margin-KM & \bf ALPS & \bf TPC & \bf {\ours~(Ours)} \\ \midrule
% 80.4\std3.0	82.9\std1.6	86.8\std2.0
% 82.2\std3.0	85.0\std1.6	87.2\std0.6
% 78.6\std2.1	81.8\std3.6	87.9\std1.0
% 79.2\std1.9	84.9\std1.5	88.6\std2.0
% 74.7\std3.3	82.6\std2.4	87.6\std0.9
% 76.7\std4.0	83.9\std2.0	88.1\std0.9
% 82.2\std3.4	86.3\std0.6	87.7\std1.0
% 83.3\std2.9	84.1\std1.1	88.2\std1.4
% 85.9\std1.9	87.4\std1.5	89.6\std0.4
{IMDB} & {2} 
&  81.8\std2.5 &	82.4\std1.7&	79.6\std1.6&	81.7\std1.3&	85.5\std1.1&	\underline{86.0\std1.2}	&83.5\std2.6	&84.5\std0.9&\bf	86.5\std0.9 \\
{Yelp-F} & {5} 
& 48.9\std1.3	& 46.6\std0.9	& 47.9\std0.6 &	45.5\std1.0 &	46.0\std1.5 &	47.5\std1.1 &	47.0\std1.0	& \underline{49.8\std0.5}	&\bf  50.5\std0.8$^{*}$ \\ 
{AG News} & {4} 
& 83.1\std1.2	& 82.8\std2.0	& 81.4\std1.0	& 84.9\std0.9	& 85.1\std1.5	& 84.6\std1.7 &	{84.2\std0.8} & 	\underline{85.6\std1.0} &\bf	86.8\std0.3$^{**}$\\
{Yahoo! Ans.} & {10} 
&  58.5\std4.0 &	55.0\std3.0 &	54.0\std1.5 &	61.4\std1.8 &	55.3\std2.1 &	57.8\std2.6 &\underline{61.9\std0.9} &	57.0\std1.6 &\bf	63.2\std1.2$^{*}$ \\
{DBPedia} & {14} 
&  89.1\std3.0 &	77.9\std2.8 &	58.9\std1.3 &	94.1\std1.4 &	92.0\std0.6 &	90.6\std0.7 &	91.2\std2.8 &\underline{94.3\std0.5} &\bf 95.4\std0.4$^{**}$\\
{TREC} & {6} 
&  69.4\std2.8 &	66.4\std3.5 &	41.6\std2.5 &	68.1\std2.3 &	61.0\std4.6 &	64.8\std2.7 &	\underline{72.1\std2.3} &	59.5\std3.3 &\bf 76.1\std1.1$^{**}$ \\
\midrule
{Average} &  --- &
71.9 &	68.6&	60.4	&72.6&	71.0	&71.9	& \underline{73.2} &	71.8& \textbf{76.5}~\scriptsize{\blue{($\uparrow$ 3.3)}} \\
\bottomrule
\end{tabular}
}
\caption{Experimental result for prompt-based learning~\cite{gao2021making} with 32 labels as the labeling budget. The results with 64 labels are deferred to Appendix~\ref{app:prompt_64}.
}
\label{tab:lmbff_result}
% }
\vspace{-2ex}
\end{table*}


==> tables/ood.tex <==
\begin{table}[t]
% \resizebox{\linewidth}{!}{%
% \scalebox{0.57}{
\centering 
\renewcommand\arraystretch{0.8}
\fontsize{7}{9}\selectfont 
\setlength{\tabcolsep}{0.5em}
\resizebox{0.86\linewidth}{!}{%
\begin{tabular}{l|c|c|c}
% \Xhline{2\arrayrulewidth}
\toprule
\multicolumn{1}{c|}{{\bf Datasets}}   &    \multicolumn{1}{c|}{SST-2} & \multicolumn{1}{c|}{IMDB-CS} & \multicolumn{1}{c}{IMDB-CAD} \\ 
\specialrule{.4pt}{1pt}{1pt}
Random & 76.2\std2.4 &	76.4\std4.4	& 80.5\std4.7  \\
Uncertainty &  78.0\std2.3& 	66.0\std4.0&	69.9\std3.1
 \\ 
CAL         & 76.2\std3.1 &		76.5\std2.9&	77.6\std3.2 \\\specialrule{.4pt}{1pt}{1pt}
BERT-KM     & 76.9\std1.3 &	75.6\std2.0&	{81.2\std2.0} \\
Coreset     & 71.6\std2.0 &	60.7\std3.4	&63.7\std4.3 \\\specialrule{.4pt}{1pt}{1pt}
Margin-KM   & 71.5\std3.4 &		61.2\std3.0&	57.5\std2.4 \\
ALPS        & \underline{78.5\std1.9}&	\underline{78.5\std2.7}	&\underline{81.8\std2.4}\\
TPC         & 77.8\std3.8 &	72.1\std5.0	&76.9\std6.1 \\\specialrule{.4pt}{1pt}{1pt}
{\ours}     & \bf 81.5\std3.0&\bf 	81.8\std2.7	&\bf  85.3\std2.2 \\
\bottomrule
\end{tabular}
}
% \vspace{-1ex}
\caption{Experimental results on OOD tasks for IMDB dataset with the budget of 32 labels. Full results are referred to Appendix~\ref{app:ood_full}.}
\label{tab:ood_main}
% }
\end{table}

